Invariance Matters: Empowering Social Recommendation via Graph Invariant Learning

Graph-based social recommendation systems have shown significant promise in enhancing recommendation performance, particularly in addressing the issue of data sparsity in user behaviors. Typically, these systems leverage Graph Neural Networks (GNNs) to capture user preferences by incorporating high-order social influences from observed social networks. However, existing graph-based social recommendations often overlook the fact that social networks are inherently noisy, containing task-irrelevant relationships that can hinder accurate user preference learning. The removal of these redundant social relations is crucial, yet it remains challenging due to the lack of ground truth. In this paper, we approach the social denoising problem from the perspective of graph invariant learning and propose a novel method, Social Graph Invariant Learning(SGIL). Specifically,SGIL aims to uncover stable user preferences within the input social graph, thereby enhancing the robustness of graph-based social recommendation systems. To achieve this goal, SGIL first simulates multiple noisy social environments through graph generators. It then seeks to learn environment-invariant user preferences by minimizing invariant risk across these environments. To further promote diversity in the generated social environments, we employ an adversarial training strategy to simulate more potential social noisy distributions. Extensive experimental results demonstrate the effectiveness of the proposed SGIL. The code is available at https://github.com/yimutianyang/SIGIR2025-SGIL.

==> Alltex/0-abs.tex <==
\begin{abstract}
Graph-based social recommender systems have demonstrated great potential in alleviating data sparsity by leveraging high-order user influence embedded in social networks. However, most existing methods rely heavily on the observed social graph, which is often noisy and includes spurious or task-irrelevant connections that can mislead user preference learning. Identifying and removing these noisy relations is crucial but challenging due to the lack of ground-truth annotations. In this paper, we approach the social denoising problem from the perspective of graph invariant learning and propose a novel method, \fullname. Specifically, \shortname~aims to uncover stable user preferences within the input social graph, thereby enhancing the robustness of graph-based social recommendation systems. To achieve this goal, \shortname~first simulates multiple noisy social environments through graph generators. It then seeks to learn environment-invariant user preferences by minimizing invariant risk across these environments. To further promote diversity in the generated social environments, we employ an adversarial training strategy to simulate more potential social noisy distributions. Extensive experimental results demonstrate the effectiveness of the proposed \shortname. The code is available at https://github.com/yimutianyang/SIGIR2025-SGIL.
\end{abstract}

==> Alltex/1-intro.tex <==
\section{Introduction}
\begin{figure*}[th]
    \centering
    \includegraphics[width=165mm]{Figures/sigir_example.pdf}
    % \vspace{-0.2cm}
    \caption{Illustration of the existing filtering-based social denoising methods and our proposed invariance-based method. Instead of filtering the noisy part of the input social graph, we encourage learning the invariant yet sufficient user preferences across environments.}
    \label{fig:intro}
    % \vspace{-0.2cm}
\end{figure*}

With the proliferation of social platforms, social recommendation has emerged as a pivotal technique for delivering personalized suggestions to users, harnessing both user-item interaction data and user-user social relationships~\cite{tang2013social}. The underlying premise is that users who are socially connected are more likely to exhibit similar preference patterns~\cite{mcpherson2001birds}. Consequently, much of the prior research has focused on how to effectively leverage the potential of social networks to enhance the learning of user preferences~\cite{ma2008sorec, konstas2009social}. Early work in this domain predominantly relied on first-order social connections to improve recommendation quality. For instance, user preferences were enhanced through social regularization~\cite{jamali2010matrix} or by incorporating trust relationships into user preference factorization~\cite{guo2015trustsvd}. These methods paved the way for more sophisticated integration of social data.



In recent years, graph-based social recommendation methods have gained prominence due to their remarkable success in improving recommendation accuracy, particularly in addressing the challenge of data sparsity within user behaviors~\cite{LightGCN, DiffNet, hu2024mgdcf}. By leveraging the powerful representational capabilities of Graph Neural Networks (GNNs), these methods encode user preferences while simultaneously capturing higher-order social influences and collaborative signals~\cite{wu2020diffnet++, DiffNet}. This has made graph-based approaches a compelling choice for incorporating social information into recommendation systems, enabling them to better model the complex relationships between users and their social networks.

However, despite the apparent benefits of aggregating all available information from social networks, many graph-based social recommendation methods fail to account for the inevitable noise inherent in these networks. Social networks are often fraught with task-irrelevant relationships that may obscure or distort the true preferences of users. Previous works~\cite{WWW2023robust, jiang2024challenging, yang2024graph} have empirically and statistically demonstrated the pervasiveness of social noise. For example, ~\cite{jiang2024challenging} defines the concept of preference-aware social homophily ratio and observes that social networks typically exhibit low homophily, meaning that social connections do not always align with user preferences. Furthermore, \cite{yang2024graph} investigates the direct use of original social networks in graph-based recommenders, revealing that such approaches result in only incremental improvements, or in some cases, a decline in performance. This highlights the importance of addressing the noise present in social data for effective recommendation learning.



Nevertheless, the task of identifying and eliminating these noisy social relations remains a substantial challenge. Current approaches typically follow a two-step paradigm: 1) filtering the social structure based on user preference signals, and 2) optimizing this filtering process using specific learning objectives, such as co-optimization~\cite{WWW2023robust, wsdm2024madm}, contrastive learning~\cite{jiang2024challenging}, and graph bottleneck learning~\cite{yang2024graph}. Although these methods have made notable strides in denoising social data, they are inherently limited by the lack of reliable mechanisms to identify and verify noise, as there are no ground truth labels available to assess the accuracy of the filtered relationships. This uncertainty raises an important question: \textbf{\emph{Given the difficulty in exhaustively removing noisy social connections, can we still learn stable and sufficient user preferences, even in the presence of noisy environments?}}



To achieve this goal, we adopt the principle of invariant learning to address the social noise issue. Invariant learning~\cite{IRM, vRex} posits that the input data contains both invariant features (stable) and spurious features (variable across different environments). The focus of invariant learning is to identify and utilize only the invariant features, thereby enhancing the model's robustness. As illustrated in Figure \ref{fig:intro}, we compare existing filtering-based social denoising methods with our proposed invariance-based approach. Drawing inspiration from this principle, we hypothesize that a task-relevant structure exists within the social graph that is both sufficient and invariant for recommendation tasks. Although this invariant structure is not directly accessible, we propose narrowing the bounds of invariance by exploring diverse noisy environments. Specifically, for a given input social graph, we first simulate multiple social environments (which embody different types of noise), and then optimize the learning objectives to encourage invariance across these environments. This formulation presents two key challenges: i) How can we simulate diverse noisy environments based on the input social networks and interactions? ii) How can we achieve invariant user preference learning across different noisy environments?

In this work, we propose a novel \fullname~, to tackle the above challenges. First, we design preference-guided environment generators that simulate multiple noisy environments, thereby approximating real-world scenarios where social noise is prevalent. Next, we capture invariant user preferences by leveraging an invariance-based regularizer. Specifically, we derive the optimization objective for each environment, taking into account the characteristics of the recommendation task, and incorporate an invariance penalty term to enforce the stability of user preferences across environments. To further ensure the diversity of the simulated noisy environments, we employ an adversarial training strategy. This strategy challenges the model iteratively, forcing it to perform well in progressively more difficult and varied environments, which ultimately improves its generalization ability.
The main contributions of this work are summarized as follows: 
\begin{itemize}[leftmargin=1.2em]
    % \item \textbf{Novel Perspective.} 
    \item We propose a novel social denoising approach \shortname~for robust recommendation from the standpoint of invariant learning. Unlike traditional methods that attempt to remove noisy data directly, \shortname~focuses on learning invariant user preferences across diverse environments, ensuring robustness despite noise. 
    % \item \textbf{Solid Methodology.} 
    \item We derive an optimization objective tailored to each social environment and design an invariance-based optimization to learn stable user preferences. Additionally, we incorporate an adversarial training strategy to guarantee the diversity of the generated environments, further enhancing the model's robustness. 
    % \item \textbf{Extensive Experiments.} 
    \item We conduct extensive experiments on three benchmark datasets. Empirical studies, including both real and semi-synthetic datasets, demonstrate the effectiveness of the proposed \shortname~method in improving social recommendation performance and robustness. 
    \end{itemize}

==> Alltex/2-related_works.tex <==
\section{Related Works}
\subsection{Graph-based Social Recommendation}
Social recommendations have been widely deployed in online services, which leverage social networks as auxiliary information to capture users' behavior patterns~\cite{marsden1993network, tang2013social}. Following the social homophily~\cite{mcpherson2001birds} and social influence theory~\cite{marsden1993network}, social recommendations are devoted to characterizing social relation effects on user preferences, including trust-based preference learning~\cite{guo2015trustsvd}, social regularization~\cite{jamali2010matrix, ma2011recommender}, and social influence modeling~\cite{DiffNet}. Early works mainly exploit shallow social relations to enhance recommendation, ignoring the complex high-order social structure influences. 
% Graph-based social recommendations have shown great progress in recent years~\cite{GraphRec, DiffNet}.  
Users' interactions can be naturally formulated in graph forms~\cite{LightGCN, yang2023generative}, many graph-based social recommendations have been proposed~\cite{DiffNet, SEPT, HGSR}. 
Particularly, borrowing the power of representation ability of GNNs, graph-based social recommendations achieved an impressive process.
The core premise of this work is that incorporating high-order social neighbors and interacted items into user preference learning enriches the available information, thereby addressing the issue of data sparsity. Current studies mainly focus on modeling social structure in Euclidean space~\cite{wu2020diffnet++, SEPT}, few attempts also explore the potential of Hyperbolic space learning~\cite{TOIS2021hypersorec, HGSR}. However, despite the effectiveness of social graph modeling, current research often overlooks the challenge of social noise. Despite the effectiveness of social graph modeling, current studies rarely notice the social noise problem. Directly using the observed social graph may lead to sub-optimal results. In this work, we propose a novel social denoising method to alleviate the effect of task-irrelevant social structures in recommendations.

% The core idea is that aggregating high-order social neighbors and interacted items into user preference learning, provides more information to alleviate the data sparsity issue. Current studies mainly focus on modeling social structure in Euclidean space~\cite{wu2020diffnet++, SEPT}, few attempts also explore the potential of Hyperbolic space learning~\cite{TOIS2021hypersorec, HGSR}. Despite the effectiveness of social graph modeling, current studies rarely notice the social noise problem. Directly using the observed social graph may lead to sub-optimal results. In this work, we propose a novel social denoising method to alleviate the effect of task-irrelevant social structures in recommendations.




\subsection{Recommendation Denoising}
% Most recommendation denoising methods focus on the implicit feedback scenarios~\cite{wang2021denoising, yang2021enhanced, he2024double}, which find the vulnerable or potential feedback. However, these label-aware denoising methods can't be directly used in social denoising, because social relations are additional information without groud-truth. Such that, researchers design social denoising methods to reduce the effect of redundant social structures~\cite{TKDE2020enhancing, WWW2023robust, jiang2024challenging, yang2024graph}. Nevertheless, current solutions focus on filtering the noisy part of social networks, but identifying the noisy part is challenging due to a lack of labels. Instead of removing the noise part directly, we focus on learning stable user preferences across diverse environments~(which are full of various noise). If the model can survive in various noisy environments, it indeed captures the invariant social structure for recommendation tasks. Thus, we introduce the invariant learning principle to tackle the social noise problem.

Recommender systems are usually built on clean label assumption, but it's hard to guarantee in real-world datasets. Therefore, recommendation denoising methods are designed to collaborative filtering~\cite{wang2021denoising, yang2021enhanced, he2024double}, multimodal recommendation~\cite{ma2024multimodal, yang2025less, hu2025modality}, and social recommendation~\cite{jiang2024challenging, wsdm2024madm, yang2024graph} scenarios.
% Current recommendation denoising methods mainly focus on the implicit feedback scenarios~\cite{wang2021denoising, yang2021enhanced, he2024double}, which find the vulnerable or potential feedback. However, these label-aware denoising methods can't be directly used in social denoising, because social relations are additional information without groud-truth. 
Specifically, researchers design social denoising methods to reduce the effect of redundant social structures~\cite{TKDE2020enhancing, WWW2023robust, jiang2024challenging, yang2024graph}. Among these, ESRF leverages the adversarial training technique to generate potential social relations and filter unstable part~\cite{TKDE2020enhancing}. GDSMR~\cite{WWW2023robust} proposes a distilled social graph based on progressive preference-guided social denoising. ShaRe~\cite{jiang2024challenging} designs a social graph rewriting method with social-enhanced contrastive learning optimization. GBSR~\cite{yang2024graph} introduces the information bottleneck principle to guide the social denoising process, which can preserve the minimal yet sufficient social structure. In summary, current solutions aim to filter out the noisy part of social networks, but identifying the noisy part is challenging due to a lack of labels. Instead of removing the noise part directly, we focus on learning stable user preferences across diverse environments~(which are full of various noise). 
If the model can survive in various noisy environments, it indeed captures the invariant social structure for recommendation tasks. 
Thus, we introduce the invariant learning principle to tackle the social noise problem.



\subsection{Invariant Learning and Applications}
Invariant learning has emerged as a promising approach to address the challenges posed by Out-Of-Distribution (OOD) generalization in machine learning~\cite{IRM, vRex, EIIL, yue2025learning}. The core idea behind invariant learning is to uncover stable feature representations that remain robust under varying environmental conditions, thereby enhancing the reliability of label prediction models. This framework is based on the assumption that the data contains both spurious and invariant features, where spurious features vary unpredictably across different environments, while invariant features remain stable and consistent. The primary objective of invariant learning methods is to optimize models using Invariant Risk Minimization (IRM) by introducing an invariance-based penalty during optimization, which discourages reliance on spurious features and encourages the model to learn stable, generalizable patterns. 
Invariant learning has been successfully applied across a wide range of machine learning tasks, including image classification~\cite{IRM, EIIL}, graph learning~\cite{li2022learning, chen2022learning, ICLR2022discovering}, and recommender systems~\cite{MM2022invariant, wang2022invariant, WWW2023invariant, WWW2024unleashing, SIGIR2024multimodality}. Especially for recommender systems, ~\cite{MM2022invariant, SIGIR2024multimodality} learn invariant multimedia representation to improve the robustness of the general and cold-start recommendation scenarios. Besides, ~\cite{wang2022invariant, WWW2023invariant} leverage the invariant learning to address popularity debiasing, and ~\cite{WWW2024unleashing} captures the invariant KG subgraph to enhance recommendations.
In this work, we introduce the invariant learning principle to the social recommendation, intending to capture stable user preferences that persist across diverse social environments. 

==> Alltex/3-prelimilaries.tex <==
\section{Preliminaries}
% \subsection{Graph-denoised Social Recommendation}
\subsection{Problem Statement}
There are two kinds of entities in fundamental social recommendation scenarios: a userset $U$~($|U|=M$) and an itemset $V$~($|V|=N$). 
Users have two kinds of behaviors, user-user social relations and user-item interactions. We use matrix $\mathbf{S} \in \mathbb{R}^{M \times M}$ to describe user-user social structure, where each element $s_{ab}=1$ if user $b$ follows user $a$, otherwise $s_{ab}=0$. Similar, we use matrix {\small{$\mathbf{R} \in \mathbb{R}^{M\times N}$}} to describe user-item interactions, where each element $\mathbf{r}_{ai}=1$ if user $a$ interacted with item $i$, otherwise $\mathbf{r}_{ai}=0$. Given user $a$, item $i$, and social relation matrix $\mathbf{S}$ as input, graph-based social recommenders aim to infer the probability user $a$ will interact with item $i$: $\hat{r_{ai}}=\mathcal{G}_{\theta}(a,i,\mathbf{S})$, where $\mathcal{G}_{\theta}$ denotes GNN formulation. Thus, the optimization objective of graph-based social recommendation is defined as follows:
\begin{flalign}
    \theta^* = \mathop{\arg\min}\limits_{\theta}\mathbb{E}_{(a,i,r_{ai})\sim \mathcal{P}} \mathcal{L}_{r}(r_{ai}; \mathcal{G}_{\theta}(a,i,\mathbf{S})),
\end{flalign}

\noindent where $\mathcal{P}$ denote distribution of training data, and $\theta$ denote GNN parameters. However, user social networks are usually noisy with redundant relations~\cite{WWW2023robust}, directly using $\mathbf{S}$ to infer interaction probability may decrease the recommendation accuracy. In this work, we focus on learning robust social structure $\mathbf{S}'$ to facilitate recommendation performance:
\begin{flalign}
    \mathbf{S}'=\mathcal{F}_{\phi}(U, \mathbf{S}),
\end{flalign}

\noindent where $\mathcal{F}_{\phi}$ denotes social denoising function with the parameters $\phi$. Consequently, the final optimization of graph-noised social recommendation is described as follows:
\begin{flalign}
    \theta^*,\phi^* = \mathop{\arg\min}\limits_{\theta, \phi}\mathbb{E}_{(a,i,r_{ai})\sim \mathcal{P}} \mathcal{L}_{r}(r_{ai}; \mathcal{G}_{\theta}(a,i,\mathcal{F}_{\phi}(U, \mathbf{S}))).
\end{flalign}


\subsection{Information Bottleneck Principle}
Information Bottleneck~(IB) is a representation learning principle in machine learning, which seeks a trade-off between data fit and reducing irrelevant information~\cite{tishby2000information, tishby2015deep}. Given input data $X$, $Z$ is the hidden representation, and $Y$ is the downstream task label, which follows the Markov Chain $<X \rightarrow Z \rightarrow Y>$. IB principle describes that an optimal representation should maintain the minimal sufficient information for the downstream tasks~\cite{tishby2015deep, saxe2019information}: 
\begin{flalign}
    Z^{*} = \mathop{\arg\max}\limits_{Z} I(Y; Z)-\beta I(X; Z),
\end{flalign}

\noindent where $I(Y; Z)$ denotes the mutual information between the hidden representation $Z$ and label $Y$, $I(X; Z)$ denotes the mutual information between the hidden representation $Z$ and input data $X$
two variables, $\beta$ is the coefficient to balance these two parts. IB principle has been widely applied in machine learning tasks, such as model robustness~\cite{wu2020GIB, wang2021revisiting}, fairness~\cite{gronowski2023classification}, and explainability~\cite{bang2021explaining}. In this work, we introduce the IB principle to robust social denoising learning, which aims to seek the minimal yet sufficient social structure for recommendation tasks. 



% Given the initialized user embeddings $\mathbf{P}^0 \in \mathbb{R}^{M \times d}$ and item embeddings $\mathbf{Q}^0 \in \mathbb{R}^{N \times d}$, graph-based social recommendation methods learn user preferences from both social influence diffusion and item interest propagation~\cite{wu2020diffnet++, liao2022sociallgn}. Specifically, user $a$'s representation is iteratively updated as follows:
% \begin{flalign}
%     \mathbf{p}^{l+1}_a=GNN(\mathbf{p}^l_a, \{\mathbf{p}^l_b|b \in \mathbf{S}_a\}, \{\mathbf{q}^l_i|i \in \mathbf{R}_a\}),
% \end{flalign}
% \noindent where $\mathbf{q}^{l+1}_a$ and $\mathbf{p}^l_a$ denote user $a$'s embeddings in ${l+1}^{th}$ and ${i}^{th}$ graph convolution layer, $$


 
% Thus, the goal of graph-based social recommendation is formulated as $\hat{\mathbf{R}}=GNN(U\cup V, \mathbf{R}, \mathbf{S})$. 
% There are many efforts to model user behaviors under graph formulation, such as hierarchical attention aggregation~\cite{wu2020diffnet++} and heterogeneous graph learning~\cite{salamat2021heterographrec}. To analyze the social effect of graph-based recommendation, we keep the model architecture the same as LightGCN. We

% In this work, we investigate the effect of social networks on graph-based recommendations. To avoid the influence of different model architectures, we implement a simple graph-based social recommendation, named LightGCN-S, which is the extension of
% LightGCN~\cite{LightGCN}. Firstly, we formulate the available data as a graph $\mathcal{G}=\{U \cup V, \mathbf{A}\}$, where $U \cup V$ denotes the set of nodes, and $\mathbf{A}$ is the adjacent matrix defined as follows:

% \begin{small}
% % \vspace{-1pt}
% \begin{flalign}\label{eq:adj_matrix}
% \mathbf{A}=\left[\begin{array}{cc}
% \mathbf{S} & \mathbf{R}\\
% \mathbf{R}^T & \mathbf{0}^{N\times N}
% \end{array}\right].
% \end{flalign}
% % \vspace{-1pt}
% \end{small}

% \noindent Given the initialized node embeddings $\mathbf{E}^0 \in \mathbb{R}^{(M+N) \times d}$, LightGCN-S iteratively updates node embeddings through multiple graph convolutions:
% % \noindent Let $\mathbf{P}^0 \in \mathbb{R}^{M \times d}$ and $\mathbf{Q}^0 \in \mathbb{R}^{N \times d}$ denote initialized user and item embeddings, where $d$ is the embedding dimension. LightGCN-S updates user and item embeddings through multiple graph convolutions:
% % Given the initialized user embeddings  and item embeddings , where d
% % node embeddings $\mathbf{E}^0$, graph-based CF methods update node embeddings through multiple graph convolutions:
% %Given the userset $U$, itemset $V$, and user-item interaction matrix {\small{$\mathbf{R} \in \mathbb{R}^{M\times N}$}}, graph based methods learn user and item representations by multiple graph convolutions, consisting of iteratively neighbor aggregation and message readout. Specifically, given the initialized node embeddings $\mathbf{E}^0$, the neighbor aggregation process is described as follows:
% \begin{small}
% \begin{flalign}\label{eq:aggregation}
% \mathbf{E}^{l+1}
% =\mathbf{D}^{-\frac{1}{2}}\mathbf{A}\mathbf{D}^{-\frac{1}{2}} \mathbf{E}^l, 
% \end{flalign}
% \end{small}

% \noindent where $\mathbf{D}$ is the degree matrix of graph $\mathcal{G}$, $\mathbf{E}^{l+1}$ and $\mathbf{E}^{l}$ denote node embeddings in ${l+1}^{th}$ and ${l}^{th}$ graph convolution layer, respectively. When stacking $L$ graph convolution layers, the final node representations can be obtained with a readout operation:
% \begin{small}
% % \vspace{-1pt}
% \begin{flalign}\label{eq:readout}
% \mathbf{E}&=Readout(\mathbf{E}^0, \mathbf{E}^1, ..., \mathbf{E}^L).
% \end{flalign}
% % \vspace{-3pt}
% \end{small}

% \noindent After obtaining the learned node representations through GCNs, LightGCN-S infers the propensity that user $a$ interacts with item $i$ by an inner product: $\hat{r}_{ai}=<e_a, e_i>$. Then, the pairwise ranking loss~\cite{UAI2009BPR} is adopted to optimize model parameters:
% \begin{small}
% \begin{equation}
%     \label{eq: loss_rec}
% 	\mathcal{L}_{rec}=\sum_{a=0}^{M-1}\sum\limits_{(i,j)\in D_a }-log\sigma(\hat{r}_{ai}-\hat{r}_{aj}) + \lambda ||\mathbf{E}^0||^2,
% \end{equation} 
% \end{small}

% \noindent where $\sigma(\cdot)$ is the sigmoid activation function, $\lambda$ is the regularization coefficient.
% {\small$D_a=\{(i,j)|i\in R_a\!\wedge\!j\not\in R_a\}$} denotes the pairwise training data for user $a$. {\small$R_a$} represents user $a$ interacted items on the training data.


% \subsection{Hilbert-Schmidt Independence Criterion~(HSIC)}
% HSIC (Hilbert-Schmidt Independence Criterion) serves as a statistical measure of dependency~\cite{gretton2005measuring}. This criterion is formulated as the Hilbert-Schmidt norm, assessing the cross-covariance operator between distributions within the Reproducing Kernel Hilbert Space (RKHS). Mathematically, given two variables $X$ and $Y$, $\text{HSIC}(X, Y)$ is defined as follows:
% \begin{small}
% \begin{equation}
%     \begin{aligned}
%     HSIC(X, Y) &= ||C_{XY}||_{hs}^2 \\
%     &= \mathbb{E}_{X,X',Y,Y'}[K_X(X,X')K_Y(Y,Y')] \\
%     &+\mathbb{E}_{X,X'}[K_X(X,X')]\mathbb{E}_{Y,Y'}[K_Y(Y,Y')] \\
%     &-2\mathbb{E}_{XY}[\mathbb{E}_{X'}[K_X(X,X')] \mathbb{E}_{Y'}[K_Y(Y,Y')]],
%     \end{aligned}
%     \label{eq: HSIC}
% \end{equation}
% \end{small}

% \noindent where $K_X$ and $K_Y$ are two kernel functions for variables $X$ and $Y$, $X'$ and $Y'$ are two independent copies of $X$ and $Y$. Given the sampled instances ${(x_i, y_i)}_{i=1}^n$ from the batch training data, the $HSIC(X,Y)$ can be estimated as:
% \begin{small}
% \begin{equation}
%     \hat{HSIC}(X,Y) = (n-1)^{-2}Tr(K_XHK_YH),
% \end{equation}
% \end{small}

% \noindent where $K_X$ and $K_Y$ are used kernel matrices~\cite{gretton2005measuring}, with elements $K_{X_{ij}}=K_X(x_i,x_j)$ and $K_{Y_{ij}}=K_Y(y_i,y_j)$, $H=\mathbf{I}-\frac{1}{n}\mathbf{1}\mathbf{1}^T$ is the centering matrix, and $Tr(\cdot)$ denotes the trace of matrix. In practice, we adopt the widely used radial basis function~(RBF)~\cite{vert2004kernel} as the kernel function:
% \begin{equation}
%     \label{eq: kernel}
%     K(x_i,x_j) = exp(-\frac{||x_i-x_j||^2}{2\sigma^2}),
% \end{equation}
% \noindent where $\sigma$ is the parameter that controls the sharpness of RBF.

==> Alltex/4-model.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=160mm]{Figures/framework.pdf}
%     \vspace{-0.2cm}
%     \caption{Illustration of our proposed \shortname~.}
%     \label{fig: framework}
% \end{figure*}



\section{The Proposed \shortname~Framework}
In this section, we introduce our proposed \fullname~framework for social denoising based recommendation. Essentially, \shortname~aims to learn the minimal yet efficient social structure to facilitate recommendation tasks, which is guaranteed by the information bottleneck principle. Next, we first give the overall optimization objective of \shortname~, then introduce how to implement each component of \shortname~in detail. Finally, we instantiate \shortname~with LightGCN-S backbone.

\subsection{Overview of \shortname}
As shown in Figure \ref{fig:intro}, we present the overall objective of our proposed \shortname~framework for the social recommendation. Instead of directly using the original social structure $\mathbf{S}$, we aim to learn a denoised yet informative social structure $\mathbf{S}'$ to enhance recommendation. Due to the lack of available prior for social denoising, we introduce user preference signals to guide social graph denoising. To guarantee the trade-off between social denoising and recommendation tasks, we optimize \shortname~via graph information bottleneck principle. Thus, the goal of \shortname~is: $Max: I(\mathbf{R}; \mathbf{S'}) - \beta I(\mathbf{S'}; \mathbf{S})$. Due to the intractability of $I(\mathbf{R}; \mathbf{S'})$, we take all nodes into an intermediary for calculation. Thus, we obtain the final optimization objective of \shortname~:
\begin{flalign}
    Max: I(\mathbf{R}; U,V,\mathbf{S'}) -\beta I(\mathbf{S'}; \mathbf{S}), 
\end{flalign}

\noindent where the first term is encouraging that the denoised social graph preserves the essential information to facilitate recommendation tasks. The second term is the compression of the original social graph, aiming to filter redundant social relations.


\begin{figure}[t]
    \centering
    \includegraphics[width=82mm]{Figures/3-framework.pdf}
    \vspace{-0.2cm}
    \caption{Overview of our proposed \shortname~framework.}
    \label{fig:intro}
\end{figure}

% Thus, the goal of \shortname~is to seek the minimal efficient social structure via graph information bottleneck:
% \begin{flalign} \label{eq: SGIB}
%     Max: I(\mathbf{R}; \mathbf{S'}) - \beta I(\mathbf{S'}; \mathbf{S}).
% \end{flalign}
% \noindent where $I(\mathbf{R}; \mathbf{S'})$ denotes the mutual information between the denoised social graph $\mathbf{S'}$ and user-item interactions $\mathbf{R}$, $I(\mathbf{S'}; \mathbf{S})$ denotes the mutual information between the denoised and the original social graph.  
% \noindent Considering that $\mathbf{R}$ and $\mathbf{S}$ are two-dimensional instances, we take all nodes into an intermediary for calculation. Thus, we obtain the final optimization objective of \shortname~:
% \begin{flalign}
%     Max: I(\mathbf{R}; U,V,\mathbf{S'}) -\beta I(\mathbf{S'}; \mathbf{S}), 
% \end{flalign}

% \noindent where the first term is encouraging that the denoised social graph preserves the essential information to facilitate recommendation tasks. The second term is the compression of the original social graph, encouraging filter redundant social relations.



\subsection{Preference-guided Social Denoising}
To achieve the above objective of \shortname~, we first need to refine the denoised social graph. The challenge is that although the social graph has noisy relations, there are no available labels to guide the denoising process. Based on social homogeneity social-connected individuals have more similar behavior similarity, we inject user preference signals into the social denoising process, i.e., users with similar preferences are more likely to have social relations.

Formally, we formulate the social denoising process as a graph edge dropout problem. Given the original social graph structure $\mathbf{S}$, the denoised one is defined as:
\begin{flalign} \label{eq: graph dropout}
    \mathbf{S'}= \mathcal{F}_{\phi}(U,\mathbf{S})=\{s_{ab} \odot \rho_{ab}\},
\end{flalign}

\noindent in which $\rho_{ab} \sim Bern(w_{ab})+\epsilon$ denotes that each edge $<u_a,u_b>$ will be dropped with the probability $1-w_{ab}+\epsilon$. Here, we add the parameter $\epsilon>0$ to represent the observation bias. 
Due to lacking prior information, we introduce task-relevant user preferences to refine social structure. 
Let $\mathbf{E}^{U} \in \mathbb{R}^{M \times d}$ denote user preference representations learned from the observed interactions, such as Matrix Factorization~\cite{PMF} and LightGCN~\cite{LightGCN}. For each observed social relation $<a,b>$, the link confidence is calculated as:
\begin{flalign} \label{eq: drop probability}
    w_{ab} = (g(\mathbf{e}_a, \mathbf{e}_b)),
\end{flalign}

\noindent where $\mathbf{e}_a$ and $\mathbf{e}_b$ denotes 
user $a$ and user $b$ preference representations, respectively. $g()$ is the fusion function, we employ MLPs to realize it. However, $\mathbf{S'}$ is not differentiable with the parameter $\rho$ of Bernoulli distribution, so we use the popular concrete relaxation method~\cite{jang2016categorical} to replace:
\begin{flalign} \label{eq: drop reparameter}
    Bern(w_{ab})=sigmoid({log(\delta/(1-\delta)+w_{ab})}/t),
\end{flalign}

\noindent where $\delta \sim U(0,1)$, and $t \in \mathbb{R^{+}}$ is the temperature parameter~(we set t=0.2 in our experiments). After re-parameterization, the discrete Bernoulli distribution is transferred to a differentiable function. 

\subsection{Maximization of $I(\mathbf{R}; U,V,\mathbf{S}')$}
Given the denoised social graph $\mathbf{S}'$, we first present how to maximize the mutual information $I(\mathbf{R}; U, V, \mathbf{S'})$, which ensures the denoised social graph satisfy recommendation tasks. Specifically, we derivate the lower bound of $I(\mathbf{R}; U,V, \mathbf{S'})$ as follows:
\begin{equation}
\begin{small}
    \begin{aligned}
         I(\mathbf{R}; U,V,\mathbf{S'}) & \overset{(a)}{=} H(\mathbf{R})-H(\mathbf{R}|U,V,\mathbf{S'})\\
    & \overset{(b)}{\geq} \sum_{a=0}^{M-1}\sum_{i=0}^{N-1}\sum_{r=0}^{1} p(r,a,i,\mathbf{S'})log(p(r|a,i,\mathbf{S'}) \\ 
    & \overset{(c)}{\geq} 
    \sum_{(a,i,j) \in \mathcal{D}}log(p(r_{ai}=1|a,i,\mathbf{S'}))+log(p(r_{ai}=0|a,j,\mathbf{S'})) \\
    & \overset{(d)}{=} \sum_{(a,i,j) \in \mathcal{D}}log(\sigma(\mathcal{G}(a,i,\mathbf{S'}))) - log(\sigma(\mathcal{G}(a,j,\mathbf{S'}))) \\
    & \overset{(e)}{\geq} \sum_{(a,i,j) \in \mathcal{D}}log(\sigma(\mathcal{G}(a,i,\mathbf{S'})-\mathcal{G}(a,j,\mathbf{S'}))),   
    \end{aligned}
    \end{small}
\end{equation}


% \end{flalign}

\noindent where $\mathcal{G}(\cdot)$ is any graph-based social recommender as we mentioned in the preliminaries, $\sigma(\cdot)$is the sigmoid activation,
$\mathcal{D}=\{(a,i,j)|r_{ai}=1 \!\wedge\! r_{aj}=0\}$ is all training data. Next, we introduce each derivation step as follows: (a) is the definition of mutual information; (b) is the non-negative property of $H(\mathbf{R})$; (c) is that $p(r|a,i,\mathbf{S'})\leq 1$, and we split all samples into observed interactions and non-observed interactions; (d) $\sigma(\mathcal{G}(a,i,\mathbf{S'}))$ is the variational approximation of $p(r_{ai}=1|a,i,\mathbf{S'})$; (e) is due to $log(\sigma(x))-log(\sigma(y)) \geq log(\sigma(x-y))$. 

According to the above derivation, we can find that the popular BPR ranking loss~\cite{UAI2009BPR} is the lower bound of mutual information $I(\mathbf{R}; U,V, \mathbf{S'})$. Therefore, we employ BPR loss as the objective of mutual information maximization.
% The derivation of $(e)$ is as follows. Let $\mathcal{G}(a,i,\mathbf{S'})=\sigma(f())$

% \begin{equation}
% \begin{aligned}
%     log(\sigma(x)) - log(\sigma(y)) &= log(\frac{1+exp(-y)}{1+exp(-x)}) \\
%     & \geq log(\frac{1}{1+exp(-x)}) \geq log(\frac{1}{1+exp(-x)exp(y)}) \\
%     &= log(\sigma(x-y)),
% \end{aligned}
% \end{equation}

% 

% of $I(\mathbf{R}; U,V,\mathbf{S'})$
% It's worth noticing that if we select one non-interacted item $j$ for a given interaction pair $<i,j>$, Eq.(14) is equal to widely used BPR ranking loss~\cite{UAI2009BPR}. As we focus on the social denoising problem, 
% in this work, we employ BPR loss to replace the maximization of $I(\mathbf{R}; U,V,\mathbf{S'})$ for fair comparisons with baselines.





\subsection{Minimization of $I(\mathbf{S'}; \mathbf{S})$}
Next, we introduce how to minimize $I(\mathbf{S'}, \mathbf{S})$, which aims to reduce the redundant social relations in the original graph. Estimating the upper bound of mutual information is an intractable problem. Although some works~\cite{alemi2016VIB, cheng2020CLUB} leverage variational techniques to estimate the upper bound, but heavily rely on the prior assumption. Therefore, we introduce Hilbert-Schmidt Independence Criterion~(HSIC~\cite{gretton2005measuring}) as the approximation of the minimization of $I(\mathbf{R}; \mathbf{S'})$.

\textbf{HSIC brief.} HSIC serves as a statistical measure of dependency~\cite{gretton2005measuring}, which is formulated as the Hilbert-Schmidt norm, assessing the cross-covariance operator between distributions within the Reproducing Kernel Hilbert Space (RKHS). Mathematically, given two variables $X$ and $Y$, $\text{HSIC}(X, Y)$ is defined as follows:
\begin{small}
\begin{equation}
    \begin{aligned}
    HSIC(X, Y) &= ||C_{XY}||_{hs}^2 \\
    &= \mathbb{E}_{X,X',Y,Y'}[K_X(X,X')K_Y(Y,Y')] \\
    &+\mathbb{E}_{X,X'}[K_X(X,X')]\mathbb{E}_{Y,Y'}[K_Y(Y,Y')] \\
    &-2\mathbb{E}_{XY}[\mathbb{E}_{X'}[K_X(X,X')] \mathbb{E}_{Y'}[K_Y(Y,Y')]],
    \end{aligned}
    \label{eq: HSIC}
\end{equation}
\end{small}

\noindent where $K_X$ and $K_Y$ are two kernel functions for variables $X$ and $Y$, $X'$ and $Y'$ are two independent copies of $X$ and $Y$. Given the sampled instances ${(x_i, y_i)}_{i=1}^n$ from the batch training data, the $HSIC(X,Y)$ can be estimated as:
\begin{small}
\begin{equation}
    \hat{HSIC}(X,Y) = (n-1)^{-2}Tr(K_XHK_YH),
\end{equation}
\end{small}

\noindent where $K_X$ and $K_Y$ are used kernel matrices~\cite{gretton2005measuring}, with elements $K_{X_{ij}}=K_X(x_i,x_j)$ and $K_{Y_{ij}}=K_Y(y_i,y_j)$, $H=\mathbf{I}-\frac{1}{n}\mathbf{1}\mathbf{1}^T$ is the centering matrix, and $Tr(\cdot)$ denotes the trace of matrix. In practice, we adopt the widely used radial basis function~(RBF)~\cite{vert2004kernel} as the kernel function:
\begin{equation}
    \label{eq: kernel}
    K(x_i,x_j) = exp(-\frac{||x_i-x_j||^2}{2\sigma^2}),
\end{equation}
\noindent where $\sigma$ is the parameter that controls the sharpness of RBF. 

\textbf{HSIC-based bottleneck learning.} Given the original and denoised social graph structures $\mathbf{S}$ and $\mathbf{S'}$, we minimize $HSIC(\mathbf{S'}; \mathbf{S})$ to replace the minimization of $I(\mathbf{S'}; \mathbf{S})$. However, social graphs are non-Euclidean data, making it difficult to measure dependency. In practice, we adopt Monte Carlo sampling~\cite{shapiro2003monte} on all the node representations for calculation:
\begin{flalign} \label{eq: sampled hsic}
    Min: HSIC(\mathbf{S'}, \mathbf{S}) = \hat{HSIC}(\mathbf{E'}_{\mathcal{B}}, \mathbf{E}_{\mathcal{B}}),
\end{flalign}

\noindent where $\mathcal{B}$ denotes the batch sampling users, $\mathbf{E'}$ and $\mathbf{E}$ denote node representations, which are learned from recommenders $\mathcal{G}_{\theta, \phi}(U,V,\mathbf{S'})$ and $\mathcal{G}_{\theta}(U,V,\mathbf{S})$. Thus, we can reduce the redundant social relations via the HSIC-based bottleneck regularization:
\begin{flalign} \label{eq: hsic loss}
   \mathcal{L}_{ib} = \hat{HSIC}(\mathbf{E'}_{\mathcal{B}}, \mathbf{E}_{\mathcal{B}}).
\end{flalign}

\subsection{Instantiating the \shortname~Framework}
In this section, we instantiate our proposed \shortname~with specific graph-based social recommender $\mathcal{G}_{\theta}(U,V,\mathbf{S})$.  To avoid the effect of different message-passing mechanisms, we implement LightGCN-S as the backbone model~(we also realize \shortname~with other backbones, refer to the generality analysis). Firstly, we formulate the available data and denoised social structure as a graph $\mathcal{G}=\{U \cup V, \mathbf{A}\}$, where $U \cup V$ denotes the set of nodes, and $\mathbf{A}$ is the adjacent matrix defined as follows:
\begin{flalign}\label{eq:adj_matrix}
\mathbf{A}=\left[\begin{array}{cc}
\mathbf{S} & \mathbf{R}\\
\mathbf{R}^T & \mathbf{0}^{N\times N}
\end{array}\right].
\end{flalign}

\noindent Given the initialized node embeddings $\mathbf{E}^0 \in \mathbb{R}^{(M+N) \times d}$, LightGCN-S updates node embeddings through multiple graph convolutions:
\begin{flalign}\label{eq:aggregation}
\mathbf{E}^{l+1}
=\mathbf{D}^{-\frac{1}{2}}\mathbf{A}\mathbf{D}^{-\frac{1}{2}} \mathbf{E}^l, 
\end{flalign}

\noindent where $\mathbf{D}$ is the degree matrix of graph $\mathcal{G}$, $\mathbf{E}^{l+1}$ and $\mathbf{E}^{l}$ denote node embeddings in ${l+1}^{th}$ and ${l}^{th}$ graph convolution layer, respectively. When stacking $L$ graph convolution layers, the final node representations can be obtained with a readout operation:
\begin{flalign}\label{eq:readout}
\mathbf{E}&=Readout(\mathbf{E}^0, \mathbf{E}^1, ..., \mathbf{E}^L).
\end{flalign}


\noindent After obtaining the learned node representations through GCNs, LightGCN-S infers the propensity that user $a$ interacts with item $i$ by an inner product: $\hat{r}_{ai}=<e_a, e_i>$. All the above process are summarized as $\hat{r}_{ai}=\mathcal{G}_{\theta}(a,i,\mathbf{S})$. 

Next, we give the illustration of graph-denoised social recommendation. We first use the initialized node embeddings to obtain user preference representations $\mathbf{P}=\mathbf{E}^0[:M]$, then achieve the denoised social structure $\mathbf{S'}$ based on preference-guided social structure learning~(section 3.2). Given the learned denoised social structure $\mathbf{S'}$, we establish graph-denoised social recommender $\hat{r}_{ai}=\mathcal{G}_{\theta, \phi}(a,i,\mathbf{S'})$. Then, we select the pairwise ranking loss~\cite{UAI2009BPR} to optimize model parameters:
% \begin{small}
\begin{equation}
    \label{eq: loss_rec}
\mathcal{L}_{rec}=\sum_{a=0}^{M-1}\sum\limits_{(i,j)\in D_a }-log\sigma(\hat{r}_{ai}-\hat{r}_{aj}) + \lambda ||\mathbf{E}^0||^2,
\end{equation} 
% \end{small}

\noindent where $\sigma(\cdot)$ is the sigmoid activation function, $\lambda$ is the regularization coefficient.
{\small$D_a=\{(i,j)|i\in R_a\!\wedge\!j\not\in R_a\}$} denotes the pairwise training data for user $a$. {\small$R_a$} represents user $a$ interacted items on the training data. Combined with the HSIC-based bottleneck regularizer, we obtain the final optimization objective:
\begin{flalign} \label{eq: all loss}
    \mathop{\arg\min}\limits_{\theta, \phi} \mathcal{L} = \mathcal{L}_{rec}+\beta \mathcal{L}_{ib},
\end{flalign}

\noindent The overall learning process of \shortname~is illustrated in Algorithm 1.

\begin{algorithm}[t]
\SetAlgoNlRelativeSize{0}
\caption{The algorithm of \shortname~}
\KwData{Userset $U$, Itemset $V$, User-item interactions $\mathbf{R}$, User-user social relations $\mathbf{S}$, and observation bias $\epsilon$}
\KwResult{Optimal graph-denoised social recommender $\mathcal{G}^{*}_{\theta, \phi}(\cdot)$}
Initialize recommender $\mathcal{G}_{\theta, \phi}$ with random weights\;

\While{not converged}{
    Sample a batch training data $\mathcal{D}$\;
    Compute social edge dropout probability via Eq.\eqref{eq: drop probability}-Eq.\eqref{eq: drop reparameter}\; 
    Refine the denoised social structure $\mathbf{S'}$ via Eq.\eqref{eq: graph dropout}\;
    Obtain node representations $\mathbf{E}'$ via $\mathcal{G}_{\theta, \phi}(U,V,\mathbf{S'})$\;
    Obtain node representations $\mathbf{E}$ via $\mathcal{G}_{\theta}(U,V,\mathbf{S})$\;
    Compute recommendation task loss $\mathcal{L}_{rec}$ via Eq.\eqref{eq: loss_rec}\;
    Compute HSIC bottleneck loss $\mathcal{L}_{ib}$ via Eq.\eqref{eq: hsic loss}\;
    Update model parameters according to Eq.\eqref{eq: all loss}\;
}
\label{alg: SGIB}
Return the optimal $\mathcal{G}^{*}_{\theta, \phi}(\cdot)$;\
\end{algorithm}

\subsection{Model Discussion}
In this section, we analyze the proposed \shortname~from model complexity and model generalization.

\subsubsection{Space Complexity}
As illustrated in Algorithm 1, the parameters of \shortname~are composed of two parts: graph-based social recommender parameters $\theta$ and social denoising parameters $\phi$. Among them, $\theta=\mathbf{E}^0$ are the general parameters equipped for backbone models~(such as LightGCN-S). $\phi$ are the parameters of MLPs, which are used to calculate the social edge confidence. Because $\phi$ are the shared parameters for all social edges, the additional parameters of \shortname~are ignorable compared with backbone models.

\subsubsection{Time Complexity}
Compared with the backbone model~(such as LightGCN-S), the additional time cost is social graph denoising and HSIC-bottleneck optimization. Social graph denoising is conducted on the observed social relations, which performs a sparse matrix. Besides, the time complexity of the HSIC-bottleneck regularizer lies in the number of the sampled nodes~(refer to Eq.\eqref{eq: sampled hsic}). In practice, we adopt a mini-batch training strategy to reduce the time cost of bottleneck learning, and the additional time cost of \shortname~is affordable.
Besides, as we remove redundant social relations, the denoised yet informative social graph makes \shortname~convergence much faster than the backbone model. Experiments also verify the efficiency of \shortname.

% The time cost of \shortname~is affordable in practice, and our proposed \shortname~is much faster convergence speed compared with backbone models~(as shown in experiments).

\subsubsection{Model Generalization}
The proposed \shortname~is designed for social denoising under graph-based social recommendation scenarios. It does not depend on specific graph-based social recommenders, such as DiffNet++~\cite{wu2020diffnet++} and SocialLGN~\cite{liao2022sociallgn}. Our proposed \shortname~is a flexible denoising framework to enhance social recommendations, we also conduct experiments on four backbones to demonstrate the generalization. Besides the backbone model, the idea of introducing the information bottleneck principle to graph denoising can also be generalized for different recommendation scenarios.

==> Alltex/5-experiments.tex <==


\section{Experiments}
In this section, we conduct extensive experiments on three real-world datasets to validate the effectiveness of our proposed \shortname~. We first introduce experimental settings, followed by recommendation performance comparisons. Finally, we give a detailed model investigation, including training efficiency, visualization of the denoised social graph, and parameter sensitivities.

\begin{table}[th]
    \centering
	\setlength{\belowcaptionskip}{5pt} %
	\caption{The statistics of three datasets.}\label{tab:statistics}
	\vspace{-0.2cm}
	\scalebox{1.0}{
    \begin{tabular}{c|c|c|c}
    \hline
    Dataset & Douban-Book & Yelp & Epinions \\ \hline
    Users & 13,024 & 19,593 & 18,202  \\ 
    Items & 22,347 & 21,266 & 47,449  \\ \hline
    Interactions & 792,062 & 450,884 & 298,173 \\ 
    Social Relations & 169,150 & 864,157 & 381,559 \\ \hline
    Interaction Density & 0.048\%  & 0.034\%  & 0.035\%  \\
    Relation Density & 0.268\% & 0.206\% & 0.115\% \\ \hline
    \end{tabular}}
    \vspace{-0.2cm}
\end{table}

\subsection{Experimental Settings}
\subsubsection{Datasets} We conduct empirical studies on three public datasets to verify the effectiveness of our proposed \shortname~, including Yelp, Epinions, and Dianping~\cite{HGSR}. All datasets involve user-user social links and user-item interactions. For the Yelp dataset, we follow the released version in~\cite{SEPT}. For epinions and dianping datasets,
we filter ratings less than 3 and keep the remaining ratings as positive feedback. After that, we sample 80\% interactions as training data, and the remaining 20\%  as test data. The detailed statistics of all datasets are summarized in Table \ref{tab:statistics}.

\begin{table*}[t]
\centering
\caption{Overall performance comparisons on three benchmarks. The best performance is highlighted in \textbf{bold} and the second is highlighted by \underline{underlines}. Impro. indicates the relative improvement of our proposed \shortname~compared to the best baseline.}
 \vspace{-2pt}
\label{tab: overall performance}
\scalebox{1.02}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline 
 & \multicolumn{4}{c|}{Douban-Book}       
 & \multicolumn{4}{c|}{Yelp}
 & \multicolumn{4}{c|}{Epinions}\\ \cline{2-13}
\multirow{-2}{*}{Models} &R@10&N@10&R@20&N@20 &R@10&N@10&R@20&N@20 &R@10&N@10&R@20&N@20  \\ \hline
% BPR-MF  & 0.0869 & 0.0949 & 0.1296 & 0.1045 & 0.1627 & 0.1142 & 0.1885 & 0.1224 & 0.2093 & 0.1291 \\ \hline
LightGCN  & 0.1039 & 0.1195 & 0.1526 & 0.1283 & 0.0698 & 0.0507 & 0.1081 & 0.0623 & 0.0432 & 0.0314 & 0.0675 & 0.0385 \\ \hline
GraphRec & 0.0971 & 0.1145 & 0.1453 & 0.1237 & 0.0672 & 0.0485 & 0.1077 & 0.0607 & 0.0436 & 0.0315 & 0.0681 & 0.0387 \\ \hline
DiffNet++ & 0.1010 & 0.1184 & 0.1489 & 0.1270 & 0.0707 & 0.0516 & 0.1114 & 0.0640 & 0.0468 & 0.0329 & 0.0727 & 0.0406 \\ \hline 
SocialLGN & 0.1034 & 0.1182 & 0.1527 & 0.1274 & 0.0681 & 0.0507 & 0.1059 & 0.0620 & 0.0416 & 0.0307 & 0.0634 & 0.0371 \\ \hline
LightGCN-S & 0.1021 & 0.1187 & 0.1506 & 0.1281 & 0.0714 & 0.0529 & 0.1126 & 0.0651 & \underline{0.0477} & \underline{0.0347} & 0.0716 & \underline{0.0417}  \\ \hline \hline
Rule-based & 0.1033 & 0.1192 & 0.1518 & 0.1289 & 0.0705 & 0.0526 & 0.1126 & 0.0652 & 0.0465 & 0.0340 & 0.0716 & 0.0414 \\ \hline 
% NeuralSparse & \\ \hline
ESRF & \underline{0.1042} & \underline{0.1199} & 0.1534 & \underline{0.1301} & 0.0718 & 0.0526 & 0.1123 & 0.0645 & 0.0462 & 0.0329 & \underline{0.0727} & 0.0406 \\ \hline
GDMSR  & 0.1026 & 0.1001 & \underline{0.1538} & 0.1245 & \underline{0.0739} & \underline{0.0535} & \underline{0.1148} & \underline{0.0658} & 0.0461 & 0.0326 & 0.0721 & 0.0414 \\ \hline

% SEPT & \underline{0.1094} & \underline{0.1300} & \underline{0.1592} & \underline{0.1382} & \underline{0.0749} & \underline{0.0553} & \underline{0.1176} & \underline{}0.0682 & 0.0457 & 0.0341 & 0.0724 & 0.0416 \\ \hline

\textbf{GBSR}  & \textbf{0.1189} & \textbf{0.1451} & \textbf{0.1694} & \textbf{0.1523} & \textbf{0.0805} & \textbf{0.0592} & \textbf{0.1243} & \textbf{0.0724} & \textbf{0.0529} & \textbf{0.0385} & \textbf{0.0793} & \textbf{0.0464} \\ \hline
\textbf{Impro.} & \textbf{14.11\%} & \textbf{21.02\%} & \textbf{10.14\%} & \textbf{17.06\%} & \textbf{8.93\%} & \textbf{10.65\%} & \textbf{8.28\%} & \textbf{10.00\%} & \textbf{10.90\%} & \textbf{10.95\%} & \textbf{9.08\%} & \textbf{11.27\%}  \\ \hline
\end{tabular}}
% \vspace{-0.2cm}
\end{table*}


\subsubsection{Baselines and Evaluation Metrics.}
To evaluate the effectiveness of our proposed \shortname~, we select state-of-the-art baselines for comparisons. Specifically, these baselines can be divided into two groups: graph-based social recommendation methods~\cite{LightGCN,GraphRec,wu2020diffnet++} and social graph denoising methods~\cite{ICML2020robust, TKDE2020enhancing, WWW2023robust}, which are list as follows:
\begin{itemize}
    \item \textbf{LightGCN}~\cite{LightGCN}: is the SOTA graph-based collaborative filtering method, which simplifies GCNs by removing the redundant feature transformation and non-linear activation components for ID-based recommendation.
    \item \textbf{LightGCN-S}: We extend LightGCN to graph-based social recommendation, that each user's neighbors include their interacted items and linked social users. LightGCN-S is a basic and lightweight model, considering our proposed \shortname~ is a model-agnostic social graph denoising method, we select LightGCN-S as the backbone model.
    \item \textbf{GraphRec}~\cite{GraphRec}: is a classic graph-based social recommendation method, it incorporates user opinions and user two kinds of graphs for preference learning.
    \item \textbf{DiffNet++}~\cite{wu2020diffnet++}: is the SOTA graph-based social recommendation method, it recursively formulates user interest propagation and social influence diffusion process with a hierarchical attention mechanism.
    \item \textbf{SocialLGN}~\cite{liao2022sociallgn}: propagates user representations on both user-item interactions graph and user-user social graph with light graph convolutional layers, and fuses them for recommendation.
    \item \textbf{Rule-based}: We follow~\cite{WWW2023robust} and remove unreliable social relations based on the similarity of the user-interacted items.
    % \item \textbf{NeuralSparse}~\cite{ICML2020robust}: NeuralSparse is a robust graph representation learning method based on graph sparsification method. It adaptively removes task-irrelevant edges based on supervised labels.
    \item \textbf{ESRF}~\cite{TKDE2020enhancing}: generates alternative social neighbors and further performs neighbor denoising with adversarial training.
    \item \textbf{GDMSR}~\cite{WWW2023robust}:  designs the robust preference-guided social denoising to enhance graph-based social recommendation, it only remains the informative social relations according to preference confidences.
\end{itemize}

As we focus on implicit recommendation scenarios, we employ two widely used ranking metrics: Recall@N and NDCG@N~\cite{gunawardana2009survey, steck2013evaluation}. Specifically, Recall@N measures the percentage of the recalled positive samples for the Top-N ranking lists. Furthermore, NDCG@N assigns higher scores for those items in the top-ranked positions. In the evaluation stage, we adopt a full-ranking strategy that views all non-interacted items as candidates to avoid biased evaluation~\cite{krichene2020sampled, zhao2020revisiting}. For each model, we repeat experiments in 5 times and report the average values.



\subsubsection{Parameter Settings.} We implement our proposed \shortname~ and backbone with Tensorflow~\footnote{https://www.tensorflow.org}. For all baselines, we follow the original settings and carefully fine-tune parameters for fair comparisons. For latent embedding based methods, we initialize their embeddings with a Gaussian distribution with a mean value of 0 and a standard variance of 0.01, and fix the embedding size to 64. For model optimization, we use Adam optimizer with a learning rate of 0.001 and a batch size of 2048. We follow the mainstream ranking-based methods~\cite{UAI2009BPR}, and randomly select 1 non-interacted item as the negative sample for pairwise ranking optimization. We search the GCN layer in $[1,2,3,4]$, the regularization parameter $\lambda$ in $[0.0001, 0.001, 0.01]$. For the observation bias, we set $\epsilon=0.5$ for all datasets.
For information bottleneck constraint coefficient $\beta$, we use grid-search with different scales over three datasets, and report detailed analysis in experiments. 


\subsection{Recommendation Performances}
\subsubsection{Overall Comparisons with Baselines.}
As shown in Table \ref{tab: overall performance}, we compare our proposed \shortname~with state-of-the-art methods on three benchmarks.  For a fair comparison, all denoising methods are conducted on the LightGCN-S backbone. Given the empirical studies, we have the following observations:
\begin{itemize}
    \item Compared with LightGCN, graph-based social recommendation methods present slight improvements under most of the datasets, i.e., DiffNet++ obtains a 2.24\% improvement on the NDCG@20 metric for Yelp dataset. However, this is not always the case, all social graph recommendations show a performance degradation on the Douban-Book dataset. While supported by social graphs, it is noteworthy that graph-based social recommendation methods do not consistently outperform LightGCN in terms of performance. These demonstrate that directly using social graphs may decrease recommendation performance, it's necessary to remove redundant social relations to enhance recommendation.
    
    \item Compared with directly using original social graphs, social denoising methods present better performances in most cases.
    This indicates that social noise is ubiquitous in real-world recommendation scenarios. All social denoising methods are implemented on LightGCN-S backbone, we find that GDMSR is the strongest baseline, which benefits from preference-guided social denoising and self-correcting curriculum learning. However, these social denoising methods don't present large-margin improvements compared with the backbone model. The reason is that simple rule or assumption based denoising methods lack of theoretical guarantee, it's hard to seek an effective trade-off between social denoising and recommendation accuracy.
    
    \item Our proposed \shortname~consistently outperforms all baselines under all experimental settings. Specifically, \shortname~ improves the strongest baseline $w.r.t$ NDCG@20 by 17.06\%, 10\% and 11.27\% on Douban-Book, Yelp, and Epinions datasets, respectively. Compared with the backbone model, \shortname~achieves impressive superiority over three benchmarks. These indicate that our proposed \shortname~ can significantly improve graph-based social recommendations, demonstrating the effectiveness of graph bottleneck learning to reduce redundant social relations. Compared with other social denoising methods, our \shortname~can better obtain the trade-off between removing social relations and recommendation tasks.
\end{itemize}

\begin{table*}[t]
    %\small
\centering
\caption{Performance comparisons of \shortname~on different backbones.}
 \vspace{-5pt}
\label{tab: different backbones}
\scalebox{1.05}{
\begin{tabular}{l|c|c|c|c|c|c}
\hline 
 & \multicolumn{2}{c|}{Douban-Book}       
 & \multicolumn{2}{c|}{Yelp}
 & \multicolumn{2}{c}{Epinions}\\ \cline{2-7}
\multirow{-2}{*}{Models} & Recall@20&NDCG@20&Recall@20&NDCG@20&Recall@20&NDCG@20\\ \hline 
GraphRec & 0.1453 & 0.1237 & 0.1077 & 0.0607 & 0.0681 & 0.0387\\
+GBSR &0.1510(+3.92\%) & 0.1306(+5.58\%) & 0.1136(+5.48\%) & 0.0662(+9.06\%) & 0.0706(+3.67\%) & 0.0403(+4.13\%)\\ \hline
DiffNet++ & 0.1489 & 0.1270 & 0.1114 & 0.0640 & 0.0727 & 0.0406 \\
+GBSR & 0.1545(+3.76\%) & 0.1334(+5.04\%) & 0.1224(+9.87\%) & 0.0721(+12.66\%) & 0.0790+(+8.67\%) & 0.0451(+11.08\%)\\ \hline
SocialLGN & 0.1537 & 0.1274 & 0.1059 & 0.0620 & 0.0634 & 0.0371 \\
+GBSR &0.1591(+3.51\%) & 0.1353(+6.20\%) &0.1152(+8.78\%)&0.0675(+8.87\%)&0.0675(+6.47\%) &0.0399(+7.55\%) \\ \hline
LightGCN-S & 0.1506 & 0.1281  & 0.1126 & 0.0651 & 0.0716 & 0.0417 \\
+GBSR & 0.1694(+12.48\%) & 0.1523(+18.89\%) & 0.1243(+10.39\%) & 0.0724(+11.21\%) & 0.0793(+10.75\%) & 0.0464(+11.27\%) \\ \hline
\end{tabular}}
\end{table*}

\subsubsection{Ablation study}
We conduct ablation studies on three datasets to explore the effectiveness of each component of the proposed \shortname~framework. As shown in Table~\ref{tab: ablation study}, we compare \shortname~with corresponding variants on Top-20 recommendation performances. \textit{GBSR}-w/o HSIC denotes that remove the HSIC-based bottleneck regularization of \shortname~, we only keep preference-guided social denoising module. From Table~\ref{tab: ablation study}, we can find that GBSR-w/o HSIC performs worse in all cases, even worse than the backbone model. This indicates that simple social structure learning without HSIC-based bottleneck regularization is useless for recommendation tasks. Furthermore, under the constraint of the information bottleneck principle, the learned social structure is meaningful, which can effectively improve social recommendations on three datasets.


\subsubsection{Generality study of \shortname~}
As we mentioned in the model discussion, the proposed \shortname~is a model-agnostic social denoising framework. 
To better illustrate the generality of \shortname~, we conduct experiments of \shortname~on several graph-based social recommendation backbones. As shown in Table \ref{tab: different backbones}, we implement \shortname~under four backbones, including GraphRec~\cite{GraphRec}, DiffNet++\cite{wu2020diffnet++}, SocialLGN~\cite{liao2022sociallgn}, and LightGCN-S, and report their performances of Top-20 recommendation task.
From Table \ref{tab: different backbones}, we observe that \shortname~consistently outperforms each backbone by a large margin. For example, on the Yelp dataset, \shortname~achieves 9.06\%, 12.66\%, 8.87\%, and 11.21\% improvements of NDCG@20 compared with GraphRec, DiffNet++, SocialLGN, and LightGCN-S, respectively. Similarly, \shortname~also obtains 5.48\%, 9.87\%, 8.78\%, and 10.39\% improvements on the Recall@20 metric.
Extensive experimental results show that our proposed \shortname~has a good generalization ability, which can easily coupled with current graph-based social recommendation methods and further enhancement. 



\subsection{Investigation of \shortname~}
In this section, we further analyze \shortname~from the following aspects: training efficiency, visualization of the denoised social graphs, and hyper-parameter sensitivity analysis.


\begin{table}[t]
    %\small
\centering
\caption{Ablation study on three datasets.}
 \vspace{-5pt}
\label{tab: ablation study}
\scalebox{0.90}{
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline 
 & \multicolumn{2}{c|}{Douban-Book}       
 & \multicolumn{2}{c|}{Yelp}
 & \multicolumn{2}{c|}{Epinions}\\ \cline{2-7}
\multirow{-2}{*}{Models} & R@20&N@20&R@20&N@20&R@20&N@20\\ \hline 
LightGCN-S & 0.1506 & 0.1281 & 0.1126 & 0.0651 & 0.0716 & 0.0417\\ \hline
\textit{GBSR}-w/o HSIC & 0.1482 & 0.1259 & 0.1119 & 0.0644 & 0.0688 & 0.0388\\ \hline
\textit{GBSR} & 0.1694 & 0.1523 & 0.1243 & 0.0724 & 0.0793 & 0.0464\\ \hline
\end{tabular}}
% \vspace{-0.2cm}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=42mm]{Figures/4-convergence_douban.pdf}
    \includegraphics[width=42mm]{Figures/5-convergence_yelp.pdf}
    \caption{Convergence curves of \shortname~and LightGCN-S on Douban-Book and Yelp datasets.}
    \label{fig:training efficiency}
\end{figure}



\subsubsection{Training efficiency of GBSR}
To analyze the training efficiency of \shortname~, we compare the convergence speed of \shortname~and corresponding backbone~(LightGCN-S).
As shown in Figure \ref{fig:training efficiency}, we compare the convergence process of both models. As the space limit, we only present the convergence process on Douban-Book and Yelp datasets. We set gcn layer to 3 and keep all experimental settings the same. According to these figures, we can observe that \shortname~converges much faster than the backbone model. Particularly, \shortname~reaches the best performances at the $82^{th}$, the $67^{th}$ epoch on Douban-Book and Yelp datasets. In contrast, LightGCN-S obtains the best results on $509^{th}$, and $261^{th}$ epoch, respectively. Empirical evidence shows that \shortname~convergence 2-3 times faster than LightGCN-S.  




\subsubsection{Visualization and statistics of the denoised social graphs}
Here we first present the visualization of the denoised social graph.
As shown in Figure \ref{fig: visualization}(a), we present the sampled ego-network from Douban-Book datasets. The red node denotes the center user of this ego-network, and the blue nodes denote social neighbors. The depth of the node color denotes the probability of edge dropping,  where the darker the color, the lower the dropping probability. We can observe that user social neighbors perform different confidences of social relations.  Besides, we analyze the statistics of the denoised social graphs. As shown in Figure \ref{fig: visualization}(b), we plot the mean and variance values of social relation confidence on three datasets. We can observe that Douban-Book presents the lowest mean value of social confidence, which means that it has the most social noise over the three datasets. This also explains the results of Figure \ref{fig: socialrec} that graph-based social recommendations show a performance decrease compared with LightGCN on the Douban-Book dataset. These results demonstrate that the proposed \shortname~can effectively refine the observed social graph via information bottleneck, which provides informative social structures to enhance social recommendations.



\subsubsection{Parameter Sensitivity Analysis.} In this part, we analyze the impact of different hyper-parameters of \shortname~. There are two key parameters, bottleneck loss coefficient $\beta$ and RBF sharpness parameter $\sigma^2$. As both parameters determine the scale of bottleneck loss, we combine them to analyze the influence of recommendation results. As shown in Figure \ref{fig: parameter sensitivity}, we conduct careful grid-search of $(\beta, \sigma^2)$ on three datasets. We can observe that \shortname~reaches the best performance when $\beta=40, \sigma^2=2.5$ on Douban-Book, $\beta=2.0, \sigma^2=0.25$ on Yelp, and $\beta=3.0, \sigma^2=0.25$, respectively.


\begin{figure}[t]
    \centering
    \subfloat[Ego-network~(from Douban-Book)]{\includegraphics[width=38mm]{Figures/6-yelp.png}}
    \subfloat[Errorbar of social relation confidence]{
    \includegraphics[width=40mm]{Figures/7-mean_var.pdf}
    }
    \caption{Visualization and statistics of the denoised social graphs.}
    \label{fig: visualization}
    % \vspace{-0.2cm}
\end{figure}


\begin{figure*}[th]
    \centering
    \subfloat[Douban-Book dataset]{\includegraphics[width=56mm]{Figures/8-douban_parameter.pdf}}
    \subfloat[Yelp dataset]{\includegraphics[width=56mm]{Figures/9-yelp_parameter.pdf}}
    \subfloat[Epinions dataset]{\includegraphics[width=56mm]{Figures/10-epinions_parameter.pdf}}
    % \vspace{-0.2cm}
    \caption{Performance comparisons under different parameters $(\beta, \sigma^2)$.}
    \label{fig: parameter sensitivity}
\end{figure*}
% \vspace{-0.2cm}



==> Alltex/6-Conclusion.tex <==
\section{Conclusion}
In this paper, we investigate graph-denoised social recommendations and propose a novel \fullname~framework. Specifically, \shortname~aims to learn the denoised yet informative social structure for recommendation tasks. To achieve this goal, we first design preference-guided social denoising, then optimize the denoising process via the information bottleneck principle. Particularly, we derive the lower bound of mutual information maximization and introduce HSIC regularization to replace mutual information minimization. Extensive experiments conducted on three benchmarks demonstrate the effectiveness of our proposed \shortname~framework, i.e., over 10\% improvements on Top-20 Recommendation. Moreover, \shortname~is a model-agnostic framework, which can be flexibly coupled with various graph-based social recommenders. In the future, we will explore more potential of leveraging the IB principle to recommendation tasks, i.e., self-supervised recommendation, fairness-aware recommendation, and LLM-enhanced recommendation.

